Route, Communicate, and Reason: Gated Routing and Adaptive Depth for Efficient Multi-Agent Reasoning

Multi-agent ensembling multiplies active parameters and inference cost without answering three basic questions: which agents to consult, how deeply a query should traverse a hierarchy of agents, and when inter-agent communication is worth its cost. We present GRADE (Gated Routing and Adaptive Depth for Efficient Reasoning), a hierarchical multi-agent system in which four lightweight learned gates jointly govern agent selection, hierarchy depth, inter-agent communication, and branch pruning. Training uses CoGRPO (Collaborative Group-Relative Policy Optimization), a novel critic-free recipe that adapts GRPO to multi-agent hierarchies and assigns a shared advantage signal to every gate and agent that participated in a rollout. Agent models are drawn from a hot-swappable Expert Registry; per-agent calibration maps allow experts to be replaced at inference time without retraining. At $\sim$17B average active parameters, GRADE outperforms all baselines on GSM8K, MMLUPro, and GPQA, surpassing the strongest baseline by 4.8 points on MMLUPro at half the active compute. On AIME-2025, where model depth dominates, GRADE remains competitive to existing frameworks. Ablations isolate the hierarchy and masked cross-attention as the largest contributors to accuracy, and show that per-agent calibration is necessary for safe hot-swapping.

==> intro.tex <==

\section{Introduction}
Modern multimodal systems spend the same computation on a trivial lookup as on a
question requiring several rounds of perception and inference. This uniformity is
convenient but wasteful: most of the cost of a fixed high budget is consumed by the
minority of queries that were already easy. A natural alternative is to treat
inference as \emph{sequential evidence acquisition under uncertainty}, spending more
only when doing so is expected to change the answer. It has survived not only many decades, but also the leap into electronic typesetting, remaining essentially unchanged. It was popularised thanks to sheets and more recently with desktop publishing software like PageMaker and Microsoft Word. A natural alternative is to treat
inference as \emph{sequential evidence acquisition under uncertainty}, spending more
only when doing so is expected to change the answer. It has survived not only many decades, but also the leap into electronic typesetting \cite{ghosh2026disentangling}, remaining essentially unchanged. It was popularised thanks to sheets and more recently with desktop publishing software like PageMaker and Microsoft Word. A natural alternative is to treat
inference as \emph{sequential evidence acquisition under uncertainty}, spending more
only when doing so is expected to change the answer. It has survived not only many decades, but also the leap into electronic typesetting, remaining essentially unchanged. \citet{tang2024evoagent} was popularised thanks to sheets and more recently with desktop publishing software like PageMaker and Microsoft Word.

A natural alternative is to treat
inference as \emph{sequential evidence acquisition under uncertainty}, spending more
only when doing so is expected to change the answer. It has survived not only many decades, but also the leap into electronic typesetting, remaining essentially unchanged. It was popularised thanks to sheets and more recently with desktop publishing software like PageMaker and Microsoft Word. Aperture instantiates this idea with three components: a typed record of evidence
gathered so far, a calibrated estimator of whether that evidence is \emph{sufficient}
to answer, and a policy that decides which action to take next or whether to stop.
The design is deliberately model-agnostic -- each specialist  is a frozen black box behind a uniform interface, so the control
layer can be studied and improved independently of any single backbone~\cite{ghosh2026disentangling}. Our code is available at \url{https://github.com/parmanu-lcs2}.

\begin{table}[t]
  \centering
  \caption{Accuracy and mean inference cost across four benchmarks. Cost is normalized to the fixed-budget baseline. Accuracy and mean inference cost across four benchmarks.}
  \label{tab:results}
  \small
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    \textbf{System} & \textbf{Params} & \textbf{Docs} & \textbf{Charts} & \textbf{Scenes} & \textbf{Cost}\\
    \midrule
    Fixed budget (large)   & 34\,B & 78.1 & 71.4 & 69.8 & 1.00\\
    Fixed budget (small)   & 8\,B  & 70.6 & 63.2 & 61.1 & 0.42\\
    Static routing         & 8\,B  & 74.9 & 67.8 & 65.4 & 0.58\\
    \textbf{Aperture (ours)} & 8\,B & \textbf{77.8} & \textbf{71.0} & \textbf{69.2} & \textbf{0.59}\\
    \bottomrule
  \end{tabular}
\end{table}
